ParallelFlow: Parallelizing Linear Transformers via Flow Discretization

We present a theoretical framework for analyzing linear attention models through matrix-valued state space models (SSMs). Our approach, Parallel Flows, provides a perspective that systematically decouples temporal dynamics from implementation constraints, enabling independent analysis of critical algorithmic components: chunking, parallelization, and information aggregation. Central to this framework is the reinterpretation of chunking procedures as computations of the flows governing system dynamics. This connection establishes a bridge to mathematical tools from rough path theory, opening the door to new insights into sequence modeling architectures. As a concrete application, we analyze DeltaNet in a generalized low-rank setting motivated by recent theoretical advances. Our methods allow us to design simple, streamlined generalizations of hardware-efficient algorithms present in the literature, and to provide completely different ones, inspired by rough paths techniques, with provably lower complexity. This dual contribution demonstrates how principled theoretical analysis can both explain existing practical methods and inspire fundamentally new computational approaches.

==> sigDelta_code.tex <==
% Reference: \cite{yang2024parallelizinglineartransformersdelta}

\lstset{
    language=Python,
    basicstyle=\ttfamily\small,
    numbers=left,
    numberstyle=\ttfamily\textcolor[rgb]{0.5,0.5,0.5}{\scriptsize},
    numbersep=8pt,
    frame=lines,
    framesep=2mm,
    breaklines=true,
    keywordstyle=\color{blue},
    commentstyle=\color[rgb]{0,0.6,0}{\itshape},
    stringstyle=\color{red},
    showstringspaces=false,
    columns=flexible,
    mathescape=true
}


\begin{figure}[h!]
\centering
\begin{lstlisting}
def chunk_sigDeltaRule(A, Alpha, B, S_0):
    '''
    Computes S_1 on the chunk [0, 1] with signature kernel method
    
    A/Alpha/B: tensors shape [L, R, d]
    S_0: tensor of shape [d, d]
    L: length, R: rank, d: dimension 

    Naive complexity: O(L^2 * R * (d^2 + R*d + L*R)))
    Parallel Complexity: O_par(L*R + d)
    Memory: O(L^2*R^2 + L*R*d + d^2)
    '''
    
    L, R, d = A.shape       
    idx = torch.arange(0, L)

    # G[s, t] = (A[s+1] - A[s]) @ B[t].T  || [L, L, R, R] || O(L^2 * R^2 * d) || O_par(d)
    G = einsum(torch.roll(A, -1, dims=0) - A, B, 's i k, t j k -> s t i j')
    # G_off_diag[t] = A[t+1] @ B[t].T || [L, R, R] || O(L * R^2 * d) || O_par(d)
    G_off_diag = einsum(torch.roll(A, -1, dims=0), B, 't i k, t j k -> t i j')

    # Initialise W and U chunk 
    A_Alpha = torch.cat([A[..., None], Alpha[..., None]], dim=-1) 
    WU = torch.where(idx[:, None, None, None] == 0, A_Alpha, 0) # [L, R, d, 2]

    diagonals = torch.zeros([3, L, R, d, 2])
    for i in range(1, 2*L - 1): # Multiply all O(---) inside by O(L)
    
        # Roll Diags || O( L * R * d ) || O_par(1)
        diagonals = torch.roll(diagonals, -1, dims=0)

        # Utils
        t = i // 2
        mask = (idx <= t) & (idx > i - L) # [L]
        
        #  Diagonal Mask || O(L^2) || O_par(1)
        mask_gram = (idx[None, :] + idx[:, None] == i-2)[..., None, None] # [L, L, 1, 1]
        # Compute gram entries on diagonal || O( L^2 * R^2 ) || O_par(1)
        G_entries = torch.sum(torch.where(mask_gram, G, 0), 0) # [L, R, R]

        # Initialise next diagonal
        if i < L: diagonals[1, 0] = A_Alpha[i]

        # Diagonals Update || O(L * R^2 * d) || O_par(R)
        temp = diagonals[0] + torch.roll(diagonals[0], -1, dims=0) - diagonals[-1]  
        temp += einsum(G_entries, WU, 't i j, t j k u -> t i k u')
        temp = torch.roll(temp, 1, dims=0)
        diagonals[1, 1:] = temp[1:]
        diagonals[1] *= mask[:, None, None, None]

        # Set WU value || O(R^2 * d) || O_par(R)
        if i % 2 == 0:
            temp = diagonals[0, t-1].clone()
            temp += einsum(G_off_diag[t-1], WU[t-1], 'i j, j k u -> i k u')
            diagonals[1, t], WU[t] = temp, temp

    W, U = WU[..., 0], WU[..., 1]

    # Compute the final value S_1 || O(L * R * d^2) || O_par(d + L * R)
    # S_1 = S_0 + ( U + (W @ S_0.T)).T @ B 
    temp = U + einsum(W, S_0, "t i k, k m -> t i m")
    S_1 = S_0 + einsum(temp, B, "t i m, t i k -> m k")
    
    return S_1
\end{lstlisting}
\caption{Pytorch code showing a simple implementation of the sigDelta algorithm.}
\label{sigDelta_code}
\end{figure}



% \begin{figure}[h!]
% \centering
% \begin{lstlisting}
% def chunk_higher_rank_sigDeltaRule(A, Alpha, B, S_0):
%     '''
%     Computes S_1 on the chunk [0, 1] with signature kernel method
    
%     A/Alpha/B: tensors shape [L, R, d]
%     S_0: tensor of shape [d, d]
%     L: length, R: rank, d: dimension 

%     Complexity: 
%     '''
    
%     L, R, d = A.shape
%     idx = torch.arange(0, L)
    
%     # G: [BT, BT, rK, rK]
%     G = torch.zeros([BT, BT, RK, RK], device=device)
%     # G_off_diag: [BT, rK, rK]
%     G_off_diag = torch.zeros([BT, RK, RK], device=device)

%     # G[s, t] = (A[s+1] - A[s]) @ B[t].T   
%     G = torch.sum((torch.roll(A, -1, dims=0) - A)[:, None, :, :, None] * B.swapaxes(-1, -2)[None, :, None, :, :], -2)
%     # G_off_diag[t] = A[t+1] @ B[t].T
%     G_off_diag = torch.sum(torch.roll(A, -1, dims=0)[:, :, :, None] * B.swapaxes(-1, -2)[:, None, :, :], -2)


%     # A_Alpha: [BT, RK, K, 2]
%     A_Alpha = torch.cat([A[:, :, :, None], Alpha[:, :, :, None]], dim=-1)

%     # Initialise W and U chunk
%     WU = torch.zeros([BT, RK, K, 2], device=device)
%     WU = torch.where(idx[:, None, None, None] == 0, A_Alpha, WU)

%     diagonal_prev = torch.zeros_like(WU)
%     diagonal_now = torch.zeros_like(WU)
%     diagonal_next = torch.zeros_like(WU)

%     for i in range(1, 2*BT - 1):
%         # Roll Diags
%         diagonal_prev = diagonal_now.clone()
%         diagonal_now = diagonal_next.clone()

%         # Utils
%         t = i // 2
%         mask = (idx <= t) & (idx > i - BT) # [BT]
%         mask_gram = (idx[None, :] + idx[:, None] == i-2)[:, :, None, None] # [BT, BT, 1, 1]

%         # Compute gram entries on diagonal
%         G_entries = torch.sum(torch.where(mask_gram, G, 0), 0) # [BT, RK, RK]


%         # Initialise next diagonal
%         value = torch.sum(torch.where(idx[:, None, None, None] == i, A_Alpha, 0), 0) # [RK, K, 2]
%         diagonal_next = torch.where(idx[:, None, None, None] == 0, value[None], diagonal_next)

%         # Diagonals Update
%         temp = diagonal_now + torch.roll(diagonal_now, -1, dims=0) - diagonal_prev  
%         temp += torch.sum(G_entries[:, :, :, None, None] * WU[:, None, :, :, :], 2)
%         temp = torch.roll(temp, 1, dims=0)

%         diagonal_next = torch.where(idx[:, None, None, None] > 0, temp, diagonal_next)
%         diagonal_next *= mask[:, None, None, None]


%         if i % 2 == 0:
%             # temp = diagonal_now.clone()
%             # temp += torch.sum(G_off_diag[:, :, :, None, None] * WU[:, None, :, :, :], 2) 
%             temp = diagonal_now + torch.sum(G_off_diag[:, :, :, None, None] * WU[:, None, :, :, :], 2) 
            
%             temp *= (idx[:, None, None, None] == t-1) # temp ~ A[t] @ B[t-1].T @ W[t-1]
%             temp = torch.roll(temp, 1, dims=0)
            
%             diagonal_next = torch.where(idx[:, None, None, None] == t, temp, diagonal_next)
%             WU = torch.where(idx[:, None, None, None] == t, temp, WU)
    

%     # Compute the final value S_1 || O(L * R * d^2) 
%     # S_1 = S_0 + ( U + (W @ S_0.T)).T @ B 
%     temp = U + einsum(W, S_0, "t i k, k m -> t i m")
%     S_1 = S_0 + einsum(temp, B, "t i m, t i k -> m k")
    
%     return S_1
% \end{lstlisting}
% \caption{Pytorch code showing a simple implementation of the algorithm.}
% \label{list_code}
% \end{figure}






